Debiasing Conditional Stochastic Optimization

In this paper, we study the conditional stochastic optimization (CSO) problem which covers a variety of applications including portfolio selection, reinforcement learning, robust learning, causal inference, etc. The sample-averaged gradient of the CSO objective is biased due to its nested structure, and therefore requires a high sample complexity for convergence. We introduce a general stochastic extrapolation technique that effectively reduces the bias. We show that for nonconvex smooth objectives, combining this extrapolation with variance reduction techniques can achieve a significantly better sample complexity than the existing bounds. Additionally, we develop new algorithms for the finite-sum variant of the CSO problem that also significantly improve upon existing results. Finally, we believe that our debiasing technique has the potential to be a useful tool for addressing similar challenges in other stochastic optimization problems.

==> oldexpt.tex <==
\vspace*{-1ex}
\section{Applications and Numerical Experiments} \label{sec:experiments}
\vspace*{-1ex}
% We now consider some common instantiations of~\ref{eq:cso}/\ref{eq:fcco} and show how the additional Assumption~\eqref{a:regularity} is satisfied implying that the improvements in sample complexity that we demonstrate in this paper are applicable to these settings. 
We demonstrate the numerical performance of our proposed algorithms through two applications: invariant logistic regression and model-agnostic meta-learning. For additional applications such as instrumental variable regression and deep average precision maximization, where also our techniques apply, please refer to Appendix~\ref{app: expts}.

% Since the core component of Assumption~\eqref{a:regularity} is the $3$rd order differentiability of $\nabla f_\xi$\footnote{Other parts of Assumption~\eqref{a:regularity} can be easily satisfied by making appropriate boundedness assumptions.}, we focus on that piece in the following.

\noindent\textbf{Invariant Risk Minimization.}
Invariant learning has wide applications in machine learning and related areas~\citep{mroueh2015learning,anselmi2016unsupervised}. Invariant logistic regression~\citep{,hu2020biased} is formulated as follows:
$$
\min_{\xx} \mathbb{E}_{\xi=(\aa,b)} [\log (1 + \exp(-b\mathbb{E}_{\eta|\xi} [\eta]^\top \xx)],
$$
where $\aa$ and $b$ represent a sample and its corresponding label, and $\eta$ is a noisy observation of the sample $\aa$. 
This first part can be considered as a CSO objective, with $f_{\xi}(y) := \log(1+\exp(-b y))$ and $g_{\eta}(\xx; \xi) := \eta^\top \xx$. As the loss $f_{\xi}\in\cC^\infty$ is smooth, our results from Sections~\ref{sec:CSO} and~\ref{sec:FCCO} are applicable. 


\begin{figure}
\begin{subfigure}{.74\textwidth}
  \centering
  \includegraphics[width=0.8\linewidth]{figures/invariant_logistic_regression.pdf}
  \caption{CSO: Large $n=50000$}
  \label{fig:ilr:1}
\end{subfigure} 
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/invariant_logistic_regression_2.pdf}
  \caption{FCCO: small $n=50$}
  \label{fig:ilr:2}
\end{subfigure}
\hfill
    \caption{Performances of algorithms and their extrapolated versions on the invariant logistic regression task. 
    Algorithms in each subplot use same amount of inner batch size in each iteration.
    }
        \label{fig:ilr}
\end{figure}

We consider drawing $\xi$ from a large set ($n=50000$) and a small set ($n=50$) as CSO and FCCO problem. In the CSO problem, we compare biased gradient methods with their extrapolated variants. In the CSO problem, we compare extrapolation based methods and MLMC based methods. The results are shown in Fig.~\ref{fig:ilr}.
The extrapolated versions of BSGD, BSpiderBoost and NestedVR consistly reach lower error than their non-extrapolated counterpart. Moreover, E-NestedVR outperforms all other extrapolated algorithms and V-MLMC, matching theory findings.


\noindent\textbf{First-order MAML.}
Over the past few years, the MAML framework~\citep{finn2017model} has become quite popular for few-shot supervised learning and meta
reinforcement learning tasks.
The first-order Model-Agnostic Meta-Learning (MAML) can be formulated mathematically as follows:
\begin{align*}
\min_{\xx} \E_{i\sim p, \cD^i_\text{query}} \ell_i\left( \E_{\cD^i_\text{supp}}(\xx - \alpha \nabla \ell_i(\xx, \cD^i_\text{supp} ) ), \cD^i_\text{query} \right)
\end{align*}
where $\alpha$ is the step size, $\cD^i_\text{supp}$ and  $\cD^i_\text{query}$ are meta-training and meta-testing data respectively and $\ell_i$ being the loss function of task $i$. % \textcolor{blue}{what is $f$ and $g$}
% In the CSO framework, $f_\xi(\xx):=\ell_i(\xx,\cD^i_\text{query})$ and $g_\eta(\xx, \xi):=\xx - \alpha \nabla \ell_i(\xx, \cD^i_\text{supp}) $ where $\xi=(i,\cD^i_\text{query})$ and $\eta=\cD^i_\text{supp}$. \textcolor{blue}{
\shiva{it will be good to spell out $f_\xi$ and $g_\eta$ here.}
In this context, lots of popular choices for $f_\xi$ are smooth. For illustration purposes, we now discuss a widely used sine-wave few-shot regression task as appearing in the work of \citet{finn2017model}.
% We use sinusoid few-shot regression problem for demonstration, .

\noindent\textbf{Sinusoid Regression.}
% \textcolor{blue}{Unclear. This seems like a contrived problem. Instead of this, can we take the general first-order MAML and state additional conditions (say on $\ell$) under which our results are applicable}
% \textcolor{blue}{Para 1: General first-order MAML with loss $\ell$} If $\ell$ satisfies ...., then our results are applicable....
% \textcolor{blue}{Para 2: Say an example using sinusoid
We consider a few-shot learning task to fit a sine wave, $A \sin(t - \phi)$, using a neural network $\Phi_{\xx}(t)$ with smooth activations, where $A$ and $\phi$ represent the unknown amplitude and phase, and $\xx$ denotes the model weight. Each task $i$ is characterized by $(A^i, \phi^i, \cD^i_\text{query})$. In the FO-MAML training process, we randomly select a task $i$, and draw training data $\eta=\cD^i_\text{supp}$.
Define the loss function for a given dataset $\cD$ as $\ell_i(\Phi_{\xx}; \cD) = \frac{1}{2} \E_{t\sim\cD} \norm{A^i\sin(t-\phi^i) - \Phi_{\xx}(t)}_2^2$. We then establish the outer function $f_i(\xx)=\ell_i(\Phi_{\xx}; \cD^i_\text{query})$ and inner function $g_\eta(\xx)=\xx - \alpha \nabla_{\xx} \ell_i(\Phi_{\xx}; \cD^i_\text{supp})$. As $f_i$ is smooth, our results are applicable.

In this experiment, the amplitude $A$ is drawn from a uniform distribution $\cU(0.1, 5)$ and the phase $\phi$ is drawn from $\cU(0, \pi)$. Both $\cD_\text{supp}$ and $\cD_\text{query}$ are independently drawn from $\cU(-5,5)$. The step size is set to $\alpha=0.01$, and the Adam meta-optimizer is used. The batch size is fixed to 10.
